Reel Life vs. Real Life: How Software Developers Share Their Daily Life through Vlogs

Software developers are turning to vlogs (video blogs) to share what a day is like to walk in their shoes. Through these vlogs developers share a rich perspective of their technical work as well their personal lives. However, does the type of activities portrayed in vlogs differ from activities developers in the industry perform? Would developers at a software company prefer to show activities to different extents if they were asked to share about their day through vlogs? To answer these questions, we analyzed 130 vlogs by software developers on YouTube and conducted a survey with 335 software developers at a large software company. We found that although vlogs present traditional development activities such as coding and code peripheral activities (11%), they also prominently feature wellness and lifestyle related activities (47.3%) that have not been reflected in previous software engineering literature. We also found that developers at the software company were inclined to share more non-coding tasks (e.g., personal projects, time spent with family and friends, and health) when asked to create a mock-up vlog to promote diversity. These findings demonstrate a shift in our understanding of how software developers are spending their time and find valuable to share publicly. We discuss how vlogs provide a more complete perspective of software development work and serve as a valuable source of data for empirical research.

==> fse_vlog2_check_arXiv 2/aliases.tex <==
\usepackage{xcolor} %
\definecolor{darkgreen}{rgb}{0.05,0.5,0.05}

\newcommand{\rc}[1]{{\color{blue}\bfseries Rini: #1}}
\newcommand{\df}[1]{{\color{darkgreen}\bfseries Denae: #1}}
\newcommand{\tz}[1]{{\color{orange}\bfseries Tom: #1}}

\newcommand{\someone}[1]{{\color{red}\bfseries TODO: #1}}
\newcommand{\status}[1]{\marginpar{\color{purple}\bfseries STATUS: #1}}



\renewenvironment{quote}{%
   \list{}{%
     \rightmargin0cm
   }
   \item\relax
}
{\endlist}

\renewenvironment{quotation}{%
   \list{}{%
     \rightmargin0cm
   }
   \item\relax
}
{\endlist}

\usepackage{framed}
\usepackage[strict]{changepage}

\definecolor{PAblue}{RGB}{0,122,204}%

\newcommand{\quo}[2]{ 
	\vspace{-0.15cm}
	\def\FrameCommand{%
		\hspace{0pt}%
		{\color{PAblue}\vrule width 2pt}%
		{\color{white}\vrule width 2pt}%
		\colorbox{white}
	}%
	\MakeFramed{\advance\hsize-\width\FrameRestore}%
	\noindent\hspace{-4.55pt}%
	\begin{adjustwidth}{}{0pt}
		\vspace{-2pt}%
		``\emph{#1}'' ({#2})
		\vspace{-3pt}
	\end{adjustwidth}\endMakeFramed%
	\vspace{-0.15cm}
}

\newcommand{\inlinequo}[2]{``\emph{#1}'' (#2)}
\newcommand{\inlinequote}[1]{``\emph{#1}''}

\newcommand{\myicon}[1]{\begin{tabular}{l}\includegraphics[width=0.05\linewidth]{#1}\end{tabular}}

\newcommand{\myiconinline}[1]{\setlength\intextsep{-3pt}\setlength\columnsep{0pt}\begin{wrapfigure}{l}{0.1\columnwidth}\includegraphics[width=0.1\columnwidth]{#1}\end{wrapfigure}}

\definecolor{boxcolor}{RGB}{238, 223, 204} %
\DeclareRobustCommand{\mybox}[2][gray!20]{%
\begin{tcolorbox}[   %
        breakable,
        left=0pt,
        right=0pt,
        top=0pt,
        bottom=0pt,
        colback=#1,
        colframe=black,
        width=\dimexpr\columnwidth\relax, 
        enlarge left by=0mm,
        boxsep=5pt,
        outer arc=4pt,
        boxrule=.5mm
        ]
        #2
\end{tcolorbox}
}



\newcommand{\RQA}{How do software vloggers present their daily routine in vlogs?\xspace}
\newcommand{\RQB}{How do industry developers self report their time spent in similar activities?\xspace}
\newcommand{\RQC}{What would industry developers find valuable to be presented about their daily life?\xspace}

\newcommand{\yt}{YouTube\xspace}
\newcommand{\gh}{GitHub\xspace}
\newcommand{\MSdevs}{LSC developers\xspace}
\newcommand{\vlogdevs}{software vloggers\xspace}
\newcommand{\pretendvlog}{mock-up vlog\xspace}
\newcommand{\pretendvlogs}{mock-up vlogs\xspace}
\newcommand{\bigcompany}{large software company\xspace}
\newcommand{\wellnessactivities}{wellness activities\xspace}

==> fse_vlog2_check_arXiv 2/lookup_table.tex <==

\lookupPut{M1_01}{1}
\lookupPut{M1_02}{2}
\lookupPut{M1_03}{3}
\lookupPut{M1_04}{4}
\lookupPut{M1_05}{5}
\lookupPut{M1_06}{6}
\lookupPut{M1_07}{7}
\lookupPut{M1_08}{8}
\lookupPut{M1_09}{9}
\lookupPut{M1_10}{10}
\lookupPut{M1_11}{11}
\lookupPut{M1_13}{12}
\lookupPut{M1_14}{13}
\lookupPut{M1_15}{14}
\lookupPut{M1_16}{15}
\lookupPut{M1_17}{16}
\lookupPut{M1_19}{17}
\lookupPut{M1_20}{18}
\lookupPut{M1_21}{19}
\lookupPut{M1_22}{20}
\lookupPut{M1_23}{21}
\lookupPut{M1_24}{22}
\lookupPut{M1_25}{23}
\lookupPut{M1_26}{24}
\lookupPut{M1_27}{25}
\lookupPut{M1_28}{26}
\lookupPut{M1_29}{27}
\lookupPut{M1_30}{28}
\lookupPut{M1_31}{29}
\lookupPut{M1_33}{30}
\lookupPut{M1_34}{31}
\lookupPut{M1_37}{32}
\lookupPut{M1_38}{33}
\lookupPut{M1_39}{34}
\lookupPut{M1_40}{35}
\lookupPut{M1_42}{36}
\lookupPut{M1_46}{37}
\lookupPut{M1_47}{38}
\lookupPut{M1_48}{39}
\lookupPut{M1_49}{40}
\lookupPut{M1_50}{41}
\lookupPut{M1_51}{42}
\lookupPut{M1_52}{43}
\lookupPut{M1_54}{44}
\lookupPut{M1_55}{45}
\lookupPut{M1_56}{46}
\lookupPut{M1_57}{47}
\lookupPut{M1_58}{48}
\lookupPut{M1_60}{49}
\lookupPut{M1_61}{50}
\lookupPut{M1_63}{51}
\lookupPut{M1_64}{52}
\lookupPut{M1_65}{53}
\lookupPut{M1_66}{54}
\lookupPut{M1_67}{55}
\lookupPut{M1_68}{56}
\lookupPut{M1_69}{57}
\lookupPut{M1_70}{58}
\lookupPut{M1_71}{59}
\lookupPut{M1_72}{60}
\lookupPut{M1_74}{61}
\lookupPut{M1_75}{62}
\lookupPut{M1_78}{63}
\lookupPut{M1_82}{64}
\lookupPut{M1_84}{65}
\lookupPut{M1_85}{66}
\lookupPut{M1_86}{67}
\lookupPut{M1_87}{68}
\lookupPut{M1_88}{69}
\lookupPut{M1_91}{70}
\lookupPut{M1_92}{71}
\lookupPut{M1_93}{72}
\lookupPut{M2_94}{73}
\lookupPut{M2_95}{74}
\lookupPut{M2_96}{75}
\lookupPut{M2_98}{76}
\lookupPut{M2_99}{77}
\lookupPut{M2_100}{78}
\lookupPut{M2_101}{79}
\lookupPut{M2_102}{80}
\lookupPut{M2_103}{81}
\lookupPut{M2_104}{82}
\lookupPut{M2_105}{83}
\lookupPut{M2_106}{84}
\lookupPut{M2_107}{85}
\lookupPut{M2_110}{86}
\lookupPut{M2_111}{87}
\lookupPut{M2_112}{88}
\lookupPut{M2_113}{89}
\lookupPut{M2_114}{90}
\lookupPut{M2_115}{91}
\lookupPut{M2_118}{92}
\lookupPut{M2_119}{93}
\lookupPut{M2_120}{94}
\lookupPut{M2_121}{95}
\lookupPut{M2_122}{96}
\lookupPut{M2_123}{97}
\lookupPut{M2_124}{98}
\lookupPut{M2_125}{99}
\lookupPut{M2_126}{100}
\lookupPut{M2_127}{101}
\lookupPut{M2_128}{102}
\lookupPut{M2_129}{103}
\lookupPut{M2_130}{104}
\lookupPut{M2_131}{105}
\lookupPut{M2_132}{106}
\lookupPut{M2_133}{107}
\lookupPut{M2_134}{108}
\lookupPut{M3_135}{109}
\lookupPut{M3_136}{110}
\lookupPut{M3_137}{111}
\lookupPut{M3_138}{112}
\lookupPut{M3_139}{113}
\lookupPut{M3_141}{114}
\lookupPut{M3_142}{115}
\lookupPut{M4_144}{116}
\lookupPut{M4_145}{117}
\lookupPut{M4_146}{118}
\lookupPut{M5_149}{119}
\lookupPut{M5_150}{120}
\lookupPut{M5_152}{121}
\lookupPut{M5_153}{122}
\lookupPut{MS_16}{123}
\lookupPut{MS_17}{124}
\lookupPut{MS_18}{125}
\lookupPut{MS_19}{126}
\lookupPut{MS_2}{127}
\lookupPut{MS_7}{128}
\lookupPut{MS_8}{129}
\lookupPut{MS_9}{130}

\lookupPut{M1}{1}
\lookupPut{M2}{2}
\lookupPut{M3}{3}
\lookupPut{M4}{4}
\lookupPut{M5}{5}
\lookupPut{M6}{6}
\lookupPut{M7}{7}
\lookupPut{M8}{8}
\lookupPut{M9}{9}
\lookupPut{M10}{10}
\lookupPut{M11}{11}
\lookupPut{M13}{12}
\lookupPut{M14}{13}
\lookupPut{M15}{14}
\lookupPut{M16}{15}
\lookupPut{M17}{16}
\lookupPut{M19}{17}
\lookupPut{M20}{18}
\lookupPut{M21}{19}
\lookupPut{M22}{20}
\lookupPut{M23}{21}
\lookupPut{M24}{22}
\lookupPut{M25}{23}
\lookupPut{M26}{24}
\lookupPut{M27}{25}
\lookupPut{M28}{26}
\lookupPut{M29}{27}
\lookupPut{M30}{28}
\lookupPut{M31}{29}
\lookupPut{M33}{30}
\lookupPut{M34}{31}
\lookupPut{M37}{32}
\lookupPut{M38}{33}
\lookupPut{M39}{34}
\lookupPut{M40}{35}
\lookupPut{M42}{36}
\lookupPut{M46}{37}
\lookupPut{M47}{38}
\lookupPut{M48}{39}
\lookupPut{M49}{40}
\lookupPut{M50}{41}
\lookupPut{M51}{42}
\lookupPut{M52}{43}
\lookupPut{M54}{44}
\lookupPut{M55}{45}
\lookupPut{M56}{46}
\lookupPut{M57}{47}
\lookupPut{M58}{48}
\lookupPut{M60}{49}
\lookupPut{M61}{50}
\lookupPut{M63}{51}
\lookupPut{M64}{52}
\lookupPut{M65}{53}
\lookupPut{M66}{54}
\lookupPut{M67}{55}
\lookupPut{M68}{56}
\lookupPut{M69}{57}
\lookupPut{M70}{58}
\lookupPut{M71}{59}
\lookupPut{M72}{60}
\lookupPut{M74}{61}
\lookupPut{M75}{62}
\lookupPut{M78}{63}
\lookupPut{M82}{64}
\lookupPut{M84}{65}
\lookupPut{M85}{66}
\lookupPut{M86}{67}
\lookupPut{M87}{68}
\lookupPut{M88}{69}
\lookupPut{M91}{70}
\lookupPut{M92}{71}
\lookupPut{M93}{72}
\lookupPut{M94}{73}
\lookupPut{M95}{74}
\lookupPut{M96}{75}
\lookupPut{M98}{76}
\lookupPut{M99}{77}
\lookupPut{M100}{78}
\lookupPut{M101}{79}
\lookupPut{M102}{80}
\lookupPut{M103}{81}
\lookupPut{M104}{82}
\lookupPut{M105}{83}
\lookupPut{M106}{84}
\lookupPut{M107}{85}
\lookupPut{M110}{86}
\lookupPut{M111}{87}
\lookupPut{M112}{88}
\lookupPut{M113}{89}
\lookupPut{M114}{90}
\lookupPut{M115}{91}
\lookupPut{M118}{92}
\lookupPut{M119}{93}
\lookupPut{M120}{94}
\lookupPut{M121}{95}
\lookupPut{M122}{96}
\lookupPut{M123}{97}
\lookupPut{M124}{98}
\lookupPut{M125}{99}
\lookupPut{M126}{100}
\lookupPut{M127}{101}
\lookupPut{M128}{102}
\lookupPut{M129}{103}
\lookupPut{M130}{104}
\lookupPut{M131}{105}
\lookupPut{M132}{106}
\lookupPut{M133}{107}
\lookupPut{M134}{108}
\lookupPut{M135}{109}
\lookupPut{M136}{110}
\lookupPut{M137}{111}
\lookupPut{M138}{112}
\lookupPut{M139}{113}
\lookupPut{M141}{114}
\lookupPut{M142}{115}
\lookupPut{M144}{116}
\lookupPut{M145}{117}
\lookupPut{M146}{118}
\lookupPut{M149}{119}
\lookupPut{M150}{120}
\lookupPut{M152}{121}
\lookupPut{M153}{122}

\lookupPut{MS16}{123}
\lookupPut{MS17}{124}
\lookupPut{MS18}{125}
\lookupPut{MS19}{126}
\lookupPut{MS2}{127}
\lookupPut{MS7}{128}
\lookupPut{MS8}{129}
\lookupPut{MS9}{130}


==> fse_vlog2_check_arXiv 2/tables/vlog_activities.tex <==
\begin{table}
\newcommand{\myactivity}[2]{\scriptsize{\color{blue}$\rightarrow$ \textbf{#1}:\ #2}}
\renewcommand{\myicon}[1]{\begin{minipage}[t]{0.1\columnwidth}\vspace{0pt}\includegraphics[width=\columnwidth]{#1}\end{minipage}}

\caption{The activity categories from the analysis pf the 130 vlogs. The activities of each category used in the survey are indicated in {\color{blue}$\rightarrow$ blue text}.}
\label{tab:vlog-activities}
\vspace{-0.5\baselineskip}

\begin{tabular}{@{}p{0.1\columnwidth}@{}p{0.9\columnwidth}@{}}
\toprule

\myicon{icons/noun_hacker_2767862.png} & \small \textsc{\textbf{Code Sessions}} \hfill  \textsc{(63 videos)}  \newline Working on code, and related activities like debugging, testing, and checking code into repository. Outside the editor, consulting external sources to problem-solve and reviewing code from juniors.

\vspace{2pt}
\myactivity{Coding}{Coding and reviewing (your or others') code}
\myactivity{Peripheral coding tasks}{Code related activities (like testing, refactoring, debugging, documentation etc.)}
\myactivity{Problem solving}{Investigating and designing a solution to a problem}

\\[-3pt]
\myicon{icons/noun_Work_3497804.png} & \small \textsc{\textbf{Unspecified Work}} \hfill \textsc{(54 videos)}\newline
Parts of video capturing developers at work without specifically disclosing the activities or codes, tools etc. Typically a time-lapse recording of the workspace.

\\[-3pt]
\myicon{icons/noun_administrative_506650.png} & \small \textsc{\textbf{Administrative Tasks}} \hfill \textsc{(19 videos)} \newline %
Preparing for and conducting interviews, mentoring interns and juniors, meeting and discussing with designers and architects. For freelance and remote developers, logging work time and handling clients.

\vspace{2pt}
\myactivity{Administrative work}{Doing administrative tasks like scheduling and organizing events and meetings}
\myactivity{Mentoring}{Mentoring and helping others around you}

\\[-3pt]
\myicon{icons/noun_organize_1519532.png} & \small \textsc{\textbf{Managing work/Planning the day}} \hfill \textsc{(34 videos)}\newline 
Organizing their workday on paper or apps, working with project management software like JIRA.

\vspace{2pt}
\myactivity{Organize}{Finding and using apps to increase productivity, make collaboration easier, organizing your day etc.}

\\[-3pt]
\myicon{icons/noun_Meeting_1603366.png} & \small \textsc{\textbf{Meetings}} \hfill \textsc{(65 videos)}\newline	
Attending and leading various meetings, presenting demonstrations in some meetings.

\vspace{2pt}
\myactivity{Meetings}{Having meetings (planned or unplanned) and hallway chats}

\\[-3pt]
\myicon{icons/noun_collaboration_3215610.png} & \small \textsc{\textbf{Collaboration}}\hfill \textsc{(41 videos)}\newline	
Working with immediate team members, designers, marketing team etc. Communicating with co-workers either in-person or through emails and messages.

\vspace{2pt}
\myactivity{Networking}{Networking with people outside of circle, building your personal brand}
\myactivity{Messaging}{Talking to colleagues through video calls, emails and messages}

\\[-3pt]
\myicon{icons/noun_Learning_3475260.png} & \small \textsc{\textbf{Learning}} \hfill \textsc{(12 videos)}\newline	
Discussing techniques to learn skills, working on online courses on Udemy, CodeAcademy etc.

\\[-3pt]
\myicon{icons/noun_creative_3049475.png} & \small \textsc{\textbf{Hobbies and Side Projects}} \hfill \textsc{(35 videos)}\newline	
Working on various technical projects (like building games and applications) and non-technical projects (like running a bakery, photography) outside of work hours, volunteering and teaching at welfare organizations.

\vspace{2pt}
\myactivity{Personal projects}{Working on your personal projects (game/app development, home improvement, music production, anything you are passionate about)}

\\[-3pt]
\myicon{icons/noun_Society_2830000.png} & \small \textsc{\textbf{Social Activities}} \hfill \textsc{(37 videos)}\newline
Spending time with family and kids at home, or with friends at social events or recreational sports.

\vspace{2pt}
\myactivity{Social}{With friends and family (game night, social hours, trips etc.)}

\\[-3pt]
\myicon{icons/noun_lifestyle_2514128.png} & \small \textsc{\textbf{Health, Workout, Lifestyle}} \hfill \textsc{(100 videos)}\newline
Working out or engaging in physical training, maintaining healthy and abundant food intakes, taking short breaks or light community games. Also practicing yoga, different mindfulness practices, and doing regular tasks like groceries and laundry.	

\vspace{2pt}
\myactivity{Lifestyle}{Lifestyle related activities (browsing through gadgets and technology, spending on home improvement and accessories, planning and travelling)}
\myactivity{Health}{Health related activities (workout, meditation)}
\myactivity{Breaks}{Taking breaks in between work} \\

\bottomrule

\end{tabular}
\end{table}

==> fse_vlog2_check_arXiv 2/utils.tex <==

\usepackage{tabularx}
\usepackage{amsmath}
\let\Bbbk\relax         %
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{algpseudocode,algorithm,algorithmicx} 
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage[ampersand]{easylist}
\usepackage{multicol}
\usepackage{multirow}

\usepackage{threeparttable}
\usepackage{tabularx}

\usepackage{rotating}
\usepackage[roman]{parnotes}
\usepackage[many]{tcolorbox}
\usepackage{soul}
\usepackage{xcolor}
\usepackage{comment}
\usepackage{subcaption}
\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{verbatim}

\usepackage{xspace}
\xspaceaddexceptions{]\}}

\usepackage{hyperref}
\usepackage{array}
\usepackage[inline]{enumitem}
\usepackage[export]{adjustbox}
\usepackage{longfbox}
\usepackage{commath}
\usepackage[normalem]{ulem}
\usepackage{mdframed,lipsum}
\usepackage{ifdraft}
\usepackage{balance}

\usepackage{makecell}

\usepackage{wrapfig}

\newif\ifdraft
\drafttrue %
\newcommand{\boldification}[1]{\ifdraft \indent **\textbf{#1}** \\\indent\else\relax\fi}




